Connect, Not Collapse: Explaining Contrastive Learning for Unsupervised Domain Adaptation

We consider unsupervised domain adaptation (UDA), where labeled data from a source domain (e.g., photographs) and unlabeled data from a target domain (e.g., sketches) are used to learn a classifier for the target domain. Conventional UDA methods (e.g., domain adversarial training) learn domain-invariant features to improve generalization to the target domain. In this paper, we show that contrastive pre-training, which learns features on unlabeled source and target data and then fine-tunes on labeled source data, is competitive with strong UDA methods. However, we find that contrastive pre-training does not learn domain-invariant features, diverging from conventional UDA intuitions. We show theoretically that contrastive pre-training can learn features that vary subtantially across domains but still generalize to the target domain, by disentangling domain and class information. Our results suggest that domain invariance is not necessary for UDA. We empirically validate our theory on benchmark vision datasets.

==> Makefile <==
default: arxiv

icml:
	pdflatex main
	bibtex main
	pdflatex main

arxiv:
	pdflatex main_arxiv
	bibtex main_arxiv
	pdflatex main_arxiv

refs:
	@if [ ! -d "refdb" ]; \
	  then \
	  git clone https://github.com/percyliang/refdb;\
	fi
	cd refdb; git pull

open: default
	open -a 'Preview' main.pdf # Sorry Windows users


==> alternate_augmentation_graph_def.tex <==
\section{Defining Connectivity}
Throughout the project so far we have worked with an intuitive understanding of ``connectivity'' between class-domain pairs, but one that we haven't yet made rigorous. We have estimated this intuitive connectivity measure via domain discriminators and we have implemented a rough notion of connectivity in our simulations, but we haven't yet penned down a more complete definition that captures our intuition of domain-class pairs that are ``well-connected''. The point of this document is to lay down a few different notions of connectivity that we can more concretely discuss and hopefully turn into the definition that we use in our paper.

One difficulty in defining the connectivity between domain-class pairs is how we associate domain-class membership with augmented points. Directly inheriting the domain-class membership of the point before augmentation is ill-defined, because two distinct points can be augmented into the same point. Moreover, even if augmentations \emph{couldn't} merge two distinct points together, we intuitively want two points to ``share'' domain-class membership in augmentation space if they stem from two highly-connected domain-class pairs. The connectivity definitions described below will handle this issue in different ways.

\section{Preliminary Notation}
We employ much of the same notation from~\citet{haochen2021spectral}. Let $\natspace$ be the ``natural'' space of points, such as images without any augmentations applied. Similarly, we define $\augspace$ to be the space of augmented points. Any $\natpoint \in \natspace$ defines an augmentation distribution $\aug(x \mid \overline{x})$ over augmented points $x \in \augspace$. Between any two augmented points $x, x' \in \augspace$ we can define a notion of connectedness $w_{xx'}$ between them as

\begin{equation} \label{eq:edgeweights}
    w_{xx'} \triangleq \E_{\natpoint \sim \natspace}[\aug(x\mid\overline{x})\aug(x'\mid\overline{x})].
\end{equation}

\section{Current Simulation-Based Framework}
For each domain-class pair $dc$, we generate $N$ points in augmentation space. These augmented points inherit the domain-class assignments of their corresponding natural points (we have to ensure that all the augmented points are distinct). Then for any new natural point $\natpoint \in \natspace$ that we want to augment, we simply choose one of our existing augmented points $x$ at random and designate $x$ as the augmentation of $\natpoint$. Since we have assigned domain-class memberships to this base set of augmentations, we can define the connectivity of two domain-class pairs $(d_1c_1, d_2c_2)$ to be the probability that a natural point from $d_1c_1$ is ``augmented into'' an augmented point in $d_2c_2$ (and vice-versa). This probability is something we can easily change in the simulations to vary this notion of connectivity. The static set of augmentations (rather than considering the entire augmentation space $\augspace$) may seem forced, however, as a general definition.

\section{Modeling Uncertainty of Domain and Class Association in Augmentation Space}
Augmentations such as cropping can result in a loss of information with respect to domain and class membership. For example, random crops of two photographs of a black dog and black cat may result in two images for which it is impossible to recover the original class assignments. Blurring two photographs of a waterbird may make it hard to tell whether the bird is in water or on land. Whether desirable or not, this ambiguity is arguably what defines the connectivity between two sets of data points. In this definition of connectivity, we assume some sort of probabilistic model over domain and class membership, conditioned on an augmented data point. If a random crop $x$ of a dog painting preserves the head, then we might say $p(\text{painting-dog} \mid x) = 1$. If the crop instead only preserved a part of the body, then we could have $p(\text{painting-dog} \mid x) = p(\text{painting-cat} \mid x) = 0.5$. We can then use these domain-class probabilities conditioned on augmented images to reweight the edge weights defined in (\ref{eq:edgeweights}) to define the following connectivity measure:

\[
    \conn(d_1c_1, d_2c_2) = \sum_{x, x' \in \augspace}w_{xx'}p(d_1c_1\mid x)p(d_2c_2\mid x').
\]

If we assume the augmentation space $\augspace$ is finite, then it's easily shown that $\conn(\cdot, \cdot)$ defines a joint probability distribution over pairs of domain-class pairs.

\section{Using Domain and Class Membership in the Natural Space}
Another way to think about connectivity is by considering two distinct \emph{natural} points $\natpoint, \natpoint' \in \natspace$ and the likelihood that random augmentations take them to the same augmented point. A first pass at measuring this likelihood is the following:

\begin{equation}
    \sum_{x \in \augspace}\aug(x \mid \natpoint)\aug(x\mid\natpoint').
\end{equation}

Then we can define a connectivity measure by taking the expected value of this likelihood over all $\natpoint$ and $\natpoint'$ sampled from $d_1c_1$ and $d_2c_2$, respectively. In other words,

\[
    \conn(d_1c_1, d_2c_2) = \E_{\natpoint \sim d_1c_1, \natpoint' \sim d_2c_2}\left[\sum_{x \in \augspace}\aug(x \mid \natpoint)\aug(x\mid\natpoint')\right].
\]

To reduce notation a bit, we will actually redefine the augmentation \emph{distribution} $\aug(\cdot\mid\cdot)$ to actually be a function $\aug(\cdot) : \natspace \to \augspace$. Then for two natural points $\natpoint, \natpoint' \in \natspace$ we can write the probability that they are randomly augmented into the same point as simply

\begin{equation}
	\Prob{\aug(\natpoint) = \aug(\natpoint')}.
\end{equation}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/app_aug_conn.tex <==
\paragraph{Conversion from augmentation to positive pair distribution.}
Recall that the positive pair distribution is defined as
\begin{align}
    \pospairdist(\inputxp, \inputx) = \E_{\bar{\inputx} \sim \unlabeldist} [ \aug(\inputx \mid \bar{\inputx}) \aug(\inputxp \mid \bar{\inputx}) ].
\end{align}
The distribution $\pospairdist$ induced by $\aug$ on $\inputspace$ is
\begin{align}
    \pospairdist(\inputxp, \inputx) = \begin{cases}
        \frac{1}{8} [ \augprobr^2 + 2\augproba^2 + \augprobb^2 + 2\augprobg^2 ] &\inputxp = \inputx \\
        \frac{1}{4} [ \augprobr \augproba + \augprobb \augprobg ] &\labelx = \labelxp, \inputxp \neq \inputx \\
        \frac{1}{4} [ \augprobr \augprobb + 2 \augproba \augprobg ] &\set{\inputxp, \inputx} \in \set{\set{1, 2}, \set{3, 4}, \set{5, 6}, \set{7, 8}} \\
        \frac{1}{4} [ \augprobr \augprobg + \augproba \augprobb ] &\set{\inputxp, \inputx} \in \set{\set{1, 4}, \set{2, 3}, \set{3, 6}, \set{4, 5}, \set{5, 8}, \set{6, 7}, \set{1, 8}, \set{2, 7}}
    \end{cases}
\end{align}
and thus by the assumption that $\augprobr > \max\{\augproba, \augprobb\}$ and $\min\{\augproba, \augprobb\} > \augprobg$, the following implications hold\ks{also assume that $\augprobr, \augproba, \augprobb, \augprobg$ are all distinct}:
\begin{align}
    \augprobr > \augprobb, \augproba > \augprobg &\implies \augprobr [ \augproba - \augprobg ] > \augprobb [ \augproba - \augprobg ] \\
                                                 &\implies \pairproba / C > \pairprobg / C \\
    \augprobr > \augproba, \augprobb > \augprobg &\implies \augprobr [ \augprobb - \augprobg ] > \augproba [ \augprobb - 2\augprobg ] \\
                                                 &\implies \pairprobb / C > \pairprobg / C  \\
    \augprobr^2 + \augproba^2 + \augprobb^2 + \augprobg^2 > 2\augprobr^2 \augproba^2 + 2\augprobb^2 \augprobg^2 &\implies \augprobr^2 + 2\augproba^2 + \augprobb^2 + 2\augprobg^2 > 2\augprobr^2 \augproba^2 + 2\augprobb^2 \augprobg^2 \label{eq:follow-up-1} \\
                                                 &\implies \pairprobr / C > \pairproba / C \\
    \augprobr^2 + \augproba^2 + \augprobb^2 + \augprobg^2 > 2\augprobr^2 \augprobb^2 + 2\augproba^2 \augprobg^2 &\implies \augprobr^2 + 2\augproba^2 + \augprobb^2 + 2\augprobg^2 > 2\augprobr^2 \augprobb^2 + 2\augproba^2 \augprobg^2 \label{eq:follow-up-2} \\
                                                 &\implies \pairprobr / C > \pairprobb / C
\end{align}
where lines (\ref{eq:follow-up-1}) and (\ref{eq:follow-up-2}) use the fact that $x^2 + y^2 > 2xy$ for all $x \neq y \in \R$.



==> sections/app_simulation.tex <==
\section{Simulation Details}
\label{app:simulation}

To obtain an even more fine-grained picture, we run simulations on toy data settings, where we can precisely vary each type of connectivity, and observe:
\begin{enumerate}
	\item Sharp thresholding behavior when $\acrossdomain$ and $\acrossboth$ cross over.
	\item $\acrossdomain$ must be nontrivial.
	%\item We observe that test accuracy is high whenever $\acrossboth < \{ \acrossdomain, \acrossclass \} < \withinboth$.
\end{enumerate}

The simulation is on a finite population so that we can study the spectral decomposition directly; however, later we show empirically that these ideas still hold in real-world, continuous-population settings.
For each domain-class pair $dc$, we generate $N$ points in augmentation space. These augmented points inherit the domain-class assignments of their corresponding natural points (we have to ensure that all the augmented points are distinct). Then for any new natural point $\natpoint \in \natspace$ that we want to augment, we simply choose one of our existing augmented points $x$ at random and designate $x$ as the augmentation of $\natpoint$. Since we have assigned domain-class memberships to this base set of augmentations, we can define the connectivity of two domain-class pairs $(d_1c_1, d_2c_2)$ to be the probability that a natural point from $d_1c_1$ is ``augmented into'' an augmented point in $d_2c_2$ (and vice-versa). This probability is something we can easily change in the simulations to vary this notion of connectivity. %The static set of augmentations (rather than considering the entire augmentation space $\augspace$) may seem forced, however, as a general definition.


==> sections/reproducibility.tex <==
\section*{Reproducibility}

We detail the hyperparameters and experimental details in the paper and appendix.
We have uploaded a zipped code archive and will publish the code on Github upon acceptance.



==> sections/toy_example.tex <==
\subsection{Illustrative example: binary classification}
\label{subsec:toy-example}

\begin{figure}[tbp]
\centering
\begin{minipage}{\linewidth}
	\centering
	\includegraphics[width=\linewidth]{figs/fig2}
    \captionof{figure}{\textbf{(Left)} Illustrative example in binary classification, where each class-domain pair is a single node in the graph. Edge weights denote connectivity as in Definition~\ref{def:connectivity} (probability of sampling the endpoints as a positive pair). \textbf{(Middle)} When $\acrossdomain$ (same class, different domain) and $\acrossclass$ (different class, same domain) are greater than $\acrossboth$ (different domain, different class), the representations are oriented so that a source-trained linear classifier generalizes to the target. \textbf{(Right)} When $\acrossdomain < \acrossboth$, no linear classifier can label both the source and target correctly.}
	\label{fig:2}
\end{minipage}
\end{figure}

In this section we describe using an illustrative example how the relative magnitudes of each connectivity type influence the geometry of the learned representations.

\paragraph{Setting (Figure~\ref{fig:2}).}
Let $\numcls = 2$ and suppose that $\absolute{\cdx} = 1$ for each $c, d \in [2]$ so that the entire data distribution consists of 4 points.
For this section, denote the single point in each class-domain pair $(c, d)$ as $\cdxsingle$.
The connectivity structure is illustrated in the left panel of Figure~\ref{fig:2}, where the weight of each edge $\{\cdxsingle, \cdxosingle{c'}{d'}\}$ denotes $\conn(\cdxsingle, \cdxosingle{c'}{d'})$.

% Note: I removed the explicit definition of augmentation and just talked about edge weights
%Formally, the example $\datap{i,d}$ (of class $i$ and domain $d$) has augmentation given by 
%\begin{align*}
%    \aug(\datap{i,d}) =
%	\begin{cases}
%        \datap{i,d'} & \text{ w.p. } \propto \acrossdomain \\
%		\datap{j,d} & \text{ w.p. } \propto \acrossclass \\
%        \datap{j,d'} & \text{ w.p. } \propto \acrossboth \\
%        \datap{i,d} & \text{ w.p. } \propto 1 - \acrossdomain - \acrossclass - \acrossboth
%	\end{cases}
%\end{align*}
%where $j \neq i$, $d' \neq d$.
%We also assume that $\withinboth \triangleq 1 - \acrossdomain - \acrossclass - \acrossboth > \max \{ \acrossdomain, \acrossclass, \acrossboth \}$ (i.e., data augmentation is most likely to map each data point to itself) and appropriately normalize \ks{so that all probability distributions sum to 1}. %$\acrossdomain + \acrossclass + \acrossboth = 2 \withinboth (1 - \withinboth)$ so that the probabilities sum to 1.
%Thus, this distribution of data and augmentations satisfies $\abgconnect$.
%We also number the points $1 - 4$ in the following order: class 1 (source), class 1 (target), class -1 (source), class -1 (target).

\paragraph{Pre-training.}
\citet{haochen2021spectral} show that minimizing the spectral contrastive loss (given in Eq.~\ref{eq:scl}) is equivalent to computing the spectral decomposition of the adjacency matrix of the population augmentation graph.
In particular, on a population of size $\popsize$ they show that any embedding matrix $\embedding \in \mathbb{R}^{\popsize \times \embeddim}$ minimizing the contrastive loss can be decomposed as
\begin{align*}
    \embedding = \embeddinggt \cdot \text{diag}[\sqrt{\lambda_1}, \dots, \sqrt{\lambda_\embeddim}] \cdot R
\end{align*}
where the columns of $\embeddinggt \in \mathbb{R}^{\popsize \times \embeddim}$ are the top $\embeddim$ eigenvectors of the adjacency matrix (with associated eigenvalues $\lambda_i$) and $R \in \mathbb{R}^{\embeddim \times \embeddim}$ is an orthonormal matrix.
These eigenvectors are then used as the learned representations, so that the representation of example $i$ is the $\embeddim$-dimensional concatenation of the $i^{th}$ components of those eigenvectors.
Here, we assume $R$ is the identity matrix--this is without loss of generality, as any rotation can be folded into the downstream linear probe.

We compute the spectral decomposition algebraically and express the learned representations as a function of the connectivity parameters.
Agnostic of the ordering of the relevant parameters, $\embedding$ (with \textit{unordered} columns $\embedding_i$) in this toy example is:\footnote{%
We leave the eigenvectors unnormalized for ease of exposition; the normalized variants would multiply the entire vector by 1/2.}
\begin{align*}
    \embedding &= \begin{bmatrix*}[r]
        1 & 1 & 1 & 1 \\
        1 & -1 & 1 & -1 \\
        1 & 1 & -1 & -1 \\
        1 & -1 & -1 & 1 \\
    \end{bmatrix*} \cdot \text{diag}[\sqrt{\lambda_1}, \dots, \sqrt{\lambda_4}]
\end{align*}
where
\begin{align*}
\lambda_1 = \acrossdomain + \acrossclass + \acrossboth + \withinboth \quad
\lambda_2 = -\acrossdomain + \acrossclass - \acrossboth + \withinboth \\
\lambda_3 = \acrossdomain - \acrossclass - \acrossboth + \withinboth \quad
\lambda_4 = -\acrossdomain - \acrossclass + \acrossboth + \withinboth
\end{align*}
We use a representation dimension $\embeddim = 3$, so contrastive learning on this toy example discards the column of $\embedding$ with the lowest associated eigenvalue, where row $i$ is the representation of example $i$.
Intuitively, the second column of $\embedding$ functions as an indicator of the domain, the third column is an indicator for the class, and the fourth column is a ``noise'' vector (which does not generalize well).

\paragraph{Fine-tuning.}
We consider learning a linear classifier upon the pre-trained features. %as the max-margin hyperplane between the (labeled) source examples, i.e. the hyperplane at the midpoint between the first and third rows of $\embedding$, given by
%\begin{align*}
%    w = \begin{bmatrix}
%        0 & 0 & \sqrt{\lambda_3} & \sqrt{\lambda_4}
%    \end{bmatrix}^\top
%\end{align*}
When $\min\{\acrossdomain, \acrossclass\} > \acrossboth$ (or equivalently, $\min\{\lambda_2, \lambda_3\} > \lambda_4$), the learned feature space contains $\embedding_2$ and $\embedding_3$ and therefore allows simultaneously for perfect domain classification and generalization of the source linear classifier to the target--the middle panel of Figure~\ref{fig:2} illustrates this favorable case.
%The induced decision function sign($w^\top x$) correctly classifies the target examples if and only if $\lambda_3 > \lambda_4$, or equivalently, $\acrossdomain > \acrossboth$.
%The middle panel of Figure~\ref{fig:2} illustrates this favorable case, in which $\acrossdomain > \acrossboth$ and the linear classifier places a larger weight on the third feature dimension than on the fourth.
On the other hand, the right panel shows the case of $\acrossdomain < \acrossboth$, in which the target features are ``swapped'' so that each example is mapped nearby the source example of the opposite class and no linear classifier can perform well on both domains.
%The right panel shows the case where $\acrossdomain < \acrossboth$; essentially, the target is ``swapped'' so that each example is mapped nearby the source example of the opposite class.
%Note that in this example, only the second eigenvector contains domain information, and therefore the source-trained linear probe places 0 weight on that feature and generalizes to the target.

Importantly in this toy setting, whether or not the source-trained linear classifier can generalize to the target depends only on whether the condition $\min\{\acrossdomain, \acrossclass \} > \acrossboth$ holds and not on the relative magnitude of $\acrossdomain$ and $\acrossclass$.
Consequently, different classes within each domain can be very connected--more so than the same class across different domains--and target accuracy can still be high.
%To illustrate the importance of this connectivity ratio on a more fine-grained setting, we run simulations and observe sharp thresholding behavior when $\acrossboth$ surpasses $\acrossdomain$ (Figure~\ref{fig:threshold}, simulation details in Appendix~\ref{app:simulation}).


